Consistency of a Recurrent Language Model With Respect to Incomplete Decoding

Despite strong performance on a variety of tasks, neural sequence models trained with maximum likelihood have been shown to exhibit issues such as length bias and degenerate repetition. We study the related issue of receiving infinite-length sequences from a recurrent language model when using common decoding algorithms. To analyze this issue, we first define inconsistency of a decoding algorithm, meaning that the algorithm can yield an infinite-length sequence that has zero probability under the model. We prove that commonly used incomplete decoding algorithms - greedy search, beam search, top-k sampling, and nucleus sampling - are inconsistent, despite the fact that recurrent language models are trained to produce sequences of finite length. Based on these insights, we propose two remedies which address inconsistency: consistent variants of top-k and nucleus sampling, and a self-terminating recurrent language model. Empirical results show that inconsistency occurs in practice, and that the proposed methods prevent inconsistency.

==> tables_figures/consistent_bpe_morecontinuations.tex <==
\begin{table*}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lp{1.05\linewidth}}
\toprule
% \textbf{Prefix} & \textit{He had a guest @-@ starring role on the television}\\
% \textbf{nucleus} & film the website , with whom he wrote to the title of The Englishwoman 's Domestic Magazine . \eos\ \\
% \textbf{c-nucleus} & film the website , but he did not be a new sequel . \eos\ \\
% \midrule
\textbf{Prefix} & \textit{Payne was quoted as saying : " With the album}\\
\textbf{nucleus} & 's " album , " The Predious " , " The One With the Wind " , " I 've Ever 't Have You 's My Way " , " I 've Ever It  $\ldots$ \\
\textbf{c-nucleus} & 's " album , " The Predious " , " The One With the Wind " , " I 've Ever 't Have You 's My Way " \eos \\
\midrule
\textbf{Prefix} & \textit{In a 2006 interview , fellow actor Ben Whish}\\
\textbf{nucleus} & 's father , a young actor , and a romantic relationship with the show , " The One Where  $\ldots$ \\
\textbf{c-nucleus} & was the first time in the film , and was published in the same episode of the season . \eos \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables_figures/consistent_sampling.tex <==
\begin{table}[t]
\centering
\small 

\begin{tabular}{lll}
\toprule
&\multicolumn{1}{c}{\textbf{$\tanh$-RNN}} & \multicolumn{1}{c}{\textbf{LSTM-RNN}}
\\ 
\midrule
\textbf{consistent topk-2} & 0.00 $\pm$ 0.0 & 0.00 $\pm$ 0.0 \\
\textbf{consistent topk-4} & 0.00 $\pm$ 0.0 & 0.00 $\pm$ 0.0 \\
\textbf{consistent nucleus-0.2} & 0.00 $\pm$ 0.0 & 0.01 $\pm$ 0.0 \\
\textbf{consistent nucleus-0.4} & 0.00 $\pm$ 0.0 & 0.01 $\pm$ 0.0\\
\bottomrule
\end{tabular}
\caption{\label{tbl:rnn-results-consistent} Non-termination ratio ($r_L$ (\%)) of decoded sequences using consistent sampling methods.}
\end{table}

==> tables_figures/consistent_sampling_bpe.tex <==
\begin{table}[t]
\centering
\small 

\begin{tabular}{lll}
\toprule
&\multicolumn{1}{c}{\textbf{$\tanh$-RNN}} & \multicolumn{1}{c}{\textbf{LSTM-RNN}}
\\ 
\midrule
\textbf{consistent topk-2} & 0.00 $\pm$ 0.0 & 0.00 $\pm$ 0.01 \\
\textbf{consistent topk-4} & 0.00 $\pm$ 0.0 & 0.00 $\pm$ 0.0 \\
\textbf{consistent nucleus-0.2} & 0.04 $\pm$ 0.02 & 0.01 $\pm$ 0.01 \\
\textbf{consistent nucleus-0.4} & 0.02 $\pm$ 0.02 & 0.01 $\pm$ 0.01\\
\bottomrule
\end{tabular}
\caption{\label{tbl:rnn-results-consistent} Non-termination ratio ($r_L$ (\%)) of decoded sequences using consistent sampling methods (BPE tokenization).}
\end{table}

==> tables_figures/strnn_word_morecontinuations.tex <==
\begin{table*}[t]
\centering

\resizebox{\linewidth}{!}{
\small
\begin{tabular}{lp{1.05\linewidth}}
\toprule
\textbf{Prefix} & \textit{In his " \unk\ with Francis \unk\ " series of}\\
\textbf{Baseline} & the song , " The \unk\ " , " The \unk\ " , " The \unk\ " , " The \unk\ " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Avalanche " , " The Tallest Man " , " The Avalanche " , " The Tallest Man " , " The Avalanche " ...  \\
\textbf{STRLM} & the same name , the song was released in the United States on November 18 , 2003 . \\
\midrule
\textbf{Prefix} & \textit{Tú " as one of the most important songs on} \\
\textbf{Baseline} & the album , and " The \unk\ " , " The \unk\ " , " The \unk\ " , " The \unk\ " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Tallest Man " , " The Avalanche " , " The Tallest Man " , " The Avalanche " , " The Tallest Man " , " The Avalanche " , " The Tallest Man " ...  \\
\textbf{STRLM} & the album , the song was released on the Billboard Hot 100 , and was certified gold by the Recording Industry Association of America ( RIAA ) . \\
\midrule
\textbf{Prefix} & \textit{Pound , who believed that the " Hellenic hardness "} \\
\textbf{Baseline} & of the poem was " \unk\ " , and " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " \unk\ " , " " \unk\ " , " \unk\ " , " " \unk\ " , " " \unk\ " , " " \unk\ " , " " \unk\ " , " " \unk\ " , ...  \\
\textbf{STRLM} & was " a \unk\ of the \unk\ of the \unk\ " . \\
\midrule
\textbf{Prefix} & \textit{Due to industrial waste and automobiles , Manila suffers from} \\
\textbf{Baseline} & the \unk\ \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , \unk\ , ...  \\
\textbf{STRLM} & the \unk\ of the \unk\ , and the \unk\ of the \unk\ \unk\ , the \unk\ of the \unk\ , and the \unk\ of the \unk\ . \\
\bottomrule
\end{tabular}
}
\caption{More example continuations from the LSTM-RNN and a self-terminating LSTM-RNN ($\epsilon=10^{-3}$, word tokenization). }
\label{tbl:examples-stlstm}
\end{table*}
